Simple and Effective Gradient-Based Tuning of Sequence-to-Sequence Models

Recent trends towards training ever-larger language models have substantially improved machine learning performance across linguistic tasks. However, the huge cost of training larger models can make tuning them prohibitively expensive, motivating the study of more efficient methods. Gradient-based hyper-parameter optimization offers the capacity to tune hyper-parameters during training, yet has not previously been studied in a sequence-to-sequence setting. We apply a simple and general gradient-based hyperparameter optimization method to sequence-to-sequence tasks for the first time, demonstrating both efficiency and performance gains over strong baselines for both Neural Machine Translation and Natural Language Understanding (NLU) tasks (via T5 pretraining). For translation, we show the method generalizes across language pairs, is more efficient than Bayesian hyper-parameter optimization, and that learned schedules for some hyper-parameters can out-perform even optimal constant-valued tuning. For T5, we show that learning hyper-parameters during pretraining can improve performance across downstream NLU tasks. When learning multiple hyper-parameters concurrently, we show that the global learning rate can follow a schedule over training that improves performance and is not explainable by the `short-horizon bias' of greedy methods \citep{wu2018}. We release the code used to facilitate further research.

==> 5_experiments.tex <==



\subsection{Guiding $\beta_1$}

In order to understand the function of guided learning we begin with a case study of a single hyperparameter, which yields a guided parameterization with only a single-dimensional degree of freedom. 
We start with $\beta_1$ as it is often useful to tune and is not complicated by the application of any schedule. In Figure \ref{fig:beta1_sweep}, we compare the evolution of $\beta_1$ over training for guided runs of differing meta-learning rates and initializations, training on the German-English language pair. The unguided baseline uses the default initialization of $0.9$. 
% \begin{figure}
% 	\centering
%     \includegraphics[width=0.5\textwidth]{draft_fig_b1_sweep.pdf}
%         \caption{Comparison of guiding $\beta_1$ over the course of training, with initialization values $[0.1,0.5,0.9]$ and meta-learning-rates [$3\text{e-}5$, $3\text{e-}4$, $3\text{e-}3$]. Baseline (no guidance) uses initialization of $0.9$ and meta-learning-rate of $0$. Loss on the development set and the learned $\beta_1$ values are shown in the top and bottom panels, respectively.}
% 	\label{fig:beta1_sweep}
% \end{figure}
\begin{wrapfigure}{r}{0.5\textwidth}
  \begin{center}
    \includegraphics[width=0.48\textwidth]{draft_fig_b1_sweep.pdf}
  \end{center}
  \caption{Comparison of guiding $\beta_1$ over the course of training, with initialization values $[0.1,0.5,0.9]$ and meta-learning-rates [$3\text{e-}5$, $3\text{e-}4$, $3\text{e-}3$]. 
  %Baseline (no guidance) uses initialization of $0.9$ and meta-learning-rate of $0$. Loss on the development set and the learned $\beta_1$ values are shown in the top and bottom panels, respectively
  }
  \label{fig:beta1_sweep}
 \end{wrapfigure}

\subsubsection{Analysis}

Figure \ref{fig:beta1_sweep} illuminates the simplicity of the $\beta_1$ guidance-loss landscape; all runs with sufficiently high meta-learning rates converge\footnote{\textit{Convergence} in this sense can be observed in the gradients of the guided parameter, which settle towards $0$ for the runs which have reached the loss-defined optimum.} to remarkably similar schedules, regardless of model or $\beta_1$ initialization. That the different guided runs end up tracing the same schedule and that schedule outperforms not only the baseline, but even a thoroughly BO-tuned constant value, seems to realize a best-case scenario for guided learning: for optimizing $\beta_1$, expensive black-box optimization can be replaced with learning an optimal schedule with little or no tuning of the meta-learning rate.
%tuning $\beta_1$ can be done away with in favor of learning a better schedule with little or no tuning of the meta-learning rate at all.

Further, the converged $\beta_1$ schedule, which gently decreases $\beta_1$ over training, suggests a reasonable explanation. At the start of training, it is useful to have a high momentum as the peculiarities of the individual batches are less important than the general trends across them.
%(due to how little the model knows and how quickly it is progressing), but
As the model becomes better and training progress levels out, it is better to be sensitive to the peculiarities of the individual training batches rather than treating them all the same. A similar reasoning motivated early explorations of learning rate decay schedules \citep{lecun1991} and has been validated recently by \citet{you2019}. Thus analyzing the results from guided learning allows us to rediscover the intuitions that originally motivated exploration of learning rate decay schedules. %In doing so, we have demonstrated how a decay schedule can be successfully applied to $\beta_1$, a hyperparameter that is frequently tuned without a decay schedule.

Additionally, the 100-run Bayesian-optimized value of $\beta_1$ is roughly a constant approximation of the learned converged schedule, which is hardly changed by further BO-optimization\footnote{See Appendix \ref{sec:appendix} for plot.}. This suggests that the \textit{true optimal value} of the hyperparameter is following a schedule, and no amount of tuning a single constant value can beat a method that even roughly approximates that schedule. For hyperparameters whose optimal values change over training, methods that produce schedules will have an edge over global tuning methods (gradient-based or otherwise).

% This suggests a more general observation: if the optimal value of a hyperparameter follows a schedule over training rather than taking a single fixed value, then any global technique that selects a single constant value is at a disadvantage to methods (like greedy gradient-based optimization) which allow hyperparameters to take on a schedule of values. Picking the best constant value will lose to much less tuned schedules that are able to roughly approximate the optimal schedule.
%See Appendix TODO for gradients of converged and non-converged runs from Figure \ref{fig:beta1_sweep}.}
% Of course this only follows if the converged schedule is actually better! In Figure \ref{fig:beta1_sweep} we show the losses of each run on the development set, and observe that all guided models outperform the baseline model. The observation that many of the guided runs achieve similar performance, despite the two orders of magnitude difference in their meta-learning rate values, demonstrates that when guided parameters converge, tuning the meta-learning rate is a much more forgiving task than tuning the parameters themselves.


% This case study has demonstrated the possibility of learning a schedule for $\beta_1$ with little or no tuning that offers significant efficiency gains over traditional multi-run static tuning, as well as performance improvement over the best tuned setup. The gradually decaying schedule learned for $\beta_1$ is reminiscent of common learning-rate decay schedules. Naturally, we now perform the same analysis on the learning rate - often the single most important hyperparameter.

\subsection{Guiding $\alpha$}

We now explore the effects of tuning the learning rate ($\alpha$) via guided learning. Unlike $\beta_1$, the learning rate typically follows a predetermined schedule. Rather than throw away the benefits of the hard-coded scheme by training the learning rate value directly, we learn a scalar on the pre-defined schedule, i.e. $\textit{effective learning rate}_t = \textit{scalar} \times \textit{schedule}_t$. 
% ###################################### appendix
% In Figure \ref{fig:lr_scalar_sweep} we show models trained on the German-English language pair, across guided runs coarsely tuning the learning rate scalar with varying meta learning rates. 
% ###################################### appendix


% ###################################### appendix
% \begin{wrapfigure}{r}{0.5\textwidth}
% 	\centering%
%     \includegraphics[width=0.48\textwidth]{draft_fig_lr_sweep.pdf}
%         \caption{Learning rate scalars, color-coded by meta-learning rate. All guided runs are initialized at 1, and applied as a scalar to the same fixed learning rate schedule.}
% 	\label{fig:lr_scalar_sweep}
%  \end{wrapfigure}
% ######################################

% \begin{figure}%[!htbp]
% 	\centering%
%     \includegraphics[width=\linewidth]{fig6_lr_sweep_applied.pdf}
%         \caption{The resulting learning rate schedules when the scalars of Figure \ref{fig:lr_scalar_sweep} are applied to the baseline learning rate schedule. The baseline scheduel is shown by \textit{untuned baseline}.}
% 	\label{fig:model_lr_sweep}
% \end{figure}

% \begin{figure}%[!htbp]
% 	\centering%
%     \includegraphics[width=\linewidth]{fig7_lr_loss.pdf}
%         \caption{The dev loss curves for the schedules shown in Figure \ref{fig:model_lr_sweep}. The runs with a high meta-learning rate do well initially but stop learning as the learning rate drops too low, so plateau earlier than the other models. The guided $3e-5$ run is cropped out well above the y-bound of the plot, and achieves a final dev loss of $1.5$.}
% 	\label{fig:lr_loss}
% \end{figure}
\subsubsection{Analysis}

It is crucial to tune the learning rate and its schedule to achieve good results \cite{Bengio2012}. Unfortunately tuning a schedule is a much more complicated task than tuning a single constant value, so in practice (including in this work), learning rate schedules are frequently borrowed from previous work. 
%The importance of the learning rate schedule coupled with the frequency with which it is copied from prior art without additional tuning implies headroom for improved performance with careful schedule tuning, gated only by the prohibitive complexity of tuning the learning rate with extant methods. 
\cite{wu2018understanding} have shown that learning the learning rate greedily is subject to a \textit{short-horizon bias}, whereby the gradient of the guidance loss drives the learning rate too low and thus fails to actually learn, yielding a worse final model. This position is supported by the results of our sweep over meta-learning rates for guiding $\alpha$ 
% (Figure \ref{fig:lr_scalar_sweep})% ### appendix ###
, in which the run with the highest meta-learning rate ($3\text{e-}3$) spikes initially and then decays quickly to convergence at a nearly static value of $1\text{e-}5$ for the rest of training. This short-horizon bias means that unlike $\beta_1$, the meta-learning rate cannot simply be set to a high-enough value for convergence, but must be tuned if it is to help performance. 

However, even with a modest sweep over meta-learning rates, we are able to substantially outperform the baseline schedule. Indeed we are even able to surpass the best result from a much more expensive Bayesian optimization of the non-guided learning rate. This suggests that tuning the meta-learning rate may still be a more pragmatic approach to optimization rather than tuning the original learning rate.


% ### appendix ###
% \subsection{Combining guided parameters}
% \begin{figure*}%[!htbp]
% 	\centering%
%     \includegraphics[width=\linewidth]{draft_fig_combo.pdf}
%         \caption{Comparing guiding runs to baseline across language-pairs (columns). Guided runs are the colored lines, the unguided baselines are black lines. The blue curves depict the guiding of the learning rate, the red that of $\beta_1$, and the purple, the combination of the two. The top row shows loss and the bottom shows accuracy on the development sets. All guided runs outperform all baseline runs in accuracy across language pairs.}
% 	\label{fig:language_pairs}
% \end{figure*}
% \begin{figure*}%[!htbp]
% 	\centering%
%     \includegraphics[width=\linewidth]{draft_fig_vizier.pdf}
%         \caption{Comparing guided runs for $\beta_1$ and learning rate in isolation and jointly, to unguided models, untuned and tuned, on the German-English language pair. The black solid line is the untuned baseline. The colored lines show a single guided run, learning the value of the variable(s) depicted at the top of the column. The dotted black lines show the best single run out of 100 produced in the course of an application of Bayesian optimization for tuning the variable(s) in question.}
% 	\label{fig:tuning}
% \end{figure*}
% ### appendix ###
Thus far we have analyzed guiding individual hyperparameters in isolation, holding the other hyperparameters constant. This simplifies the optimization problem and is helpful for analysis, but misses out on potential gains of jointly guiding parameters. 
% ### appendix ###
% In Figure \ref{fig:language_pairs}, we learn both $\beta_1$ and learning rate in a single run, setting the meta learning rate to $3\text{e-}5$ for both, and comparing against an un-guided baseline with default values across $6$ different language pairs. 
% ### appendix ###
The max BLEU scores achieved per run are shown in Table \ref{tab:combo_bleu}.

%%%%%%%%%%%%%%%%%%%%%%%% old greedy bleu scores vvvvvvv
% % \begin{table}[h]
% \begin{wraptable}{r}{8cm}
%   \caption{Comparing BLEU scores of guided runs to baseline across language pairs. Meta-learning-rate is set to $3\text{e-}5$ for all runs.}
%   \footnotesize
%   \centering
%   \begin{tabular}{c|cccccc}
%     \toprule
%     & de-en & en-de & fi-en & en-fi & lt-en & en-lt \\
%     \midrule
%     baseline & 37.6 & 36.4 & 26.5 & 18.0 & 26.9 & 11.1 \\
%     \midrule
%     $\beta_1$ & \textbf{39.0} & \textbf{38.4} & \textbf{27.7} & 18.9 & \textbf{27.2} & 11.8 \\
%     $\alpha$ & 38.8 & 38.3 & 27.0 & \textbf{19.3} & 27.1 & 11.4 \\
%     $\beta_1$ \& $\alpha$ & 38.9 & \textbf{38.4} & 26.9 & 19.2 & 27.0 & \textbf{12.0} \\

%     \bottomrule
%   \end{tabular}
%   \label{tab:combo_bleu}
% \end{wraptable}
% % deen_combo_base 37.625935
% % deen_beta1_glr3e5 39.000343
% % deen_lr_glr3e5 38.75764
% % deen_combo_glr3e5 38.86581

% % ende_combo_base 36.445904
% % ende_beta1_glr3e5 38.353165
% % ende_lr_glr3e5 38.33833
% % ende_combo_glr3e5 38.438854

% % fien_combo_base 26.521357
% % fien_beta1_glr3e5 27.66385
% % fien_lr_glr3e5 27.030636
% % fien_combo_glr3e5 26.937895

% % enfi_combo_base 18.001335
% % enfi_beta1_glr3e5 18.918892
% % enfi_lr_glr3e5 19.25152
% % enfi_combo_glr3e5 19.238531

% % lten_combo_base 26.894577
% % lten_beta1_glr3e5 27.234219
% % lten_lr_glr3e5 27.059675
% % lten_combo_glr3e5 27.034056

% % enlt_combo_base 11.092238
% % enlt_beta1_glr3e5 11.839374
% % enlt_lr_glr3e5 11.373562
% % enlt_combo_glr3e5 11.993965
%%%%%%%%%%%%%%%%%%%%%%%% old greedy bleu scores ^^^^^^^^^^^^
\begin{wraptable}{r}{8cm}
  \caption{BLEU scores of guided runs vs baseline across language pairs. Meta-learning-rate is set to $3\text{e-}5$.}
  \footnotesize
  \centering
  \begin{tabular}{c|cccccc}
    \toprule
    & de-en & en-de & fi-en & en-fi & lt-en & en-lt \\
    \midrule
    baseline & 38.6 & 37.4 & 27.2 & 18.4 & 27.3 & 11.3 \\
    \midrule
    $\beta_1$ & \textbf{39.9} & \textbf{39.4} & \textbf{28.4} & 19.4 & \textbf{28.0} & 12.1 \\
    $\alpha$ & 39.6 & \textbf{39.4} & 27.6 & \textbf{19.7} & 27.7 & 11.7 \\
    $\beta_1$ \& $\alpha$ & 39.8 & 38.8 & 27.5 & 19.6 & 27.8 & \textbf{12.2} \\

    \bottomrule
  \end{tabular}
  \label{tab:combo_bleu}
\end{wraptable}
\subsubsection{Analysis}
% deen_combo_base 38.55044937133789
% deen_beta1_glr3e5 39.86650466918945
% deen_lr_glr3e5 39.610328674316406
% deen_combo_glr3e5 39.85588455200195

% ende_combo_base 37.443843841552734
% ende_beta1_glr3e5 39.39499282836914
% ende_lr_glr3e5 39.38002014160156
% ende_combo_glr3e5 38.78788757324219

% enfi_combo_base 18.399364471435547
% enfi_beta1_glr3e5 19.36855125427246
% enfi_lr_glr3e5 19.665203094482422
% enfi_combo_glr3e5 19.590164184570312

% enlt_combo_base 11.281499862670898
% enlt_beta1_glr3e5 12.113615989685059
% enlt_lr_glr3e5 11.738256454467773
% enlt_combo_glr3e5 12.233159065246582

% fien_combo_base 27.2388973236084
% fien_beta1_glr3e5 28.397171020507812
% fien_lr_glr3e5 27.565338134765625
% fien_combo_glr3e5 27.502408981323242

% lten_combo_base 27.340240478515625
% lten_beta1_glr3e5 28.003108978271484
% lten_lr_glr3e5 27.727108001708984
% lten_combo_glr3e5 27.76233673095703
In Figure \ref{fig:language_pairs}, we observe that guided learning of $\beta_1$, $\alpha$, or the combination of the two outperforms the baseline across language pairs, which suggests that it may be possible to find ``good recipes'' which generalize across training runs, further simplifying the useful application of guiding hyperparameters. While guiding $\beta_1$ and $\alpha$ together doesn't drastically change the dynamics of their evolution compared to learning each alone, we find that in some cases the combination of the two yields better results than guiding them separately, and when tuned, they outperform the individual setups.
% One of the difficulties for per-training-run HPO when optimizing multiple hyperparameters simultaneously is disentangling correlations between concurrently tuned hyperparameters. Learning hyperparameters online offers an opportunity to turn this correlation into an advantage by allowing guided parameters to dynamically adjust to the other hyperparameters, even as those may also be changing. In our experiments combining learning $\beta_1$ and $\alpha$ we did not observe any difference in the evolution of each guided parameter compared to the single-guided-parameter setting, but we do 


\subsection{Comparing guidance to tuning}

In order to fairly evaluate the practical applicability of guiding these hyperparameters, it is necessary to compare the guided runs not just against the untuned baseline but against the best model produced by typical hyperparameter optimization schemes. This offers the opportunity to evaluate the relative utility of guidance vs tuning in terms of both absolute performance and efficiency. In Figure \ref{fig:tuning}, we compare guiding $\beta_1$, $\alpha$, and their combination against the best model (determined by the minimum of loss on the development set) produced by 100-model run of black-box optimization (BO) over the hyperparameter in question. We find that across guided-parameter settings, the non-BO-optimized guided run slightly outperforms the best BO-tuned model (Table \ref{tab:tuned}). For the setups which involve guiding $\alpha$, 
%which have more to gain from tuning due to the non-converging nature of guiding the learning rate, 
small additional gains are found in tuning the meta-learning rate with the same BO procedure.


%%%%%%%%%%%%% OLD GREEDY BLEU
% % \begin{table}[h]
% \begin{wraptable}{r}{8cm}
%   \caption{Comparing BLEU scores of guided runs to baseline and the best of $100$ Bayesian-optimized runs across language pairs. Meta-learning-rate is set to $3\text{e-}5$ for untuned guided runs, and is tuned via BO in the final row. For the guided setting, the $4$ runs correspond to the coarse meta-learning rate tuning shown in Figures \ref{fig:beta1_sweep} and \ref{fig:lr_scalar_sweep}.}
%   \footnotesize
%   \centering
%   \begin{tabular}{c|c|c|ccc}
%     \toprule
%     & BO-tuned & \# of runs & $\beta_1$ & $\alpha$ & $\beta_1$ \& $\alpha$\\
%     \midrule
%     \multirow{2}{*}{baseline} & no & 1 & 38.0 & 38.0 & 38.0 \\
%      & yes &100 & 38.6 & 38.7 & 38.8 \\
%     \midrule
%     \multirow{2}{*}{guided} & no & 4 & 39.0 & 38.8 & 38.9 \\
%     & yes &100 & 39.0 & 38.9 & \textbf{39.1} \\
%     \bottomrule
%   \end{tabular}
%   \label{tab:tuned}
% \end{wraptable}
% % combo_base_single 37.625935
% % combo_guided_single 38.86581
% % combo_base_tuned 38.837517
% % beta1_single_guided 39.11642
% % beta1_single_base 38.045662

% % beta1_tuned_base 38.561474
% % lr_single_guided 38.81545
% % lr_single_base 38.045662
% % lr_tuned_base 38.7034


% % combo_guided_tuned 39.1 https://xm2a.corp.google.com/experiments/33815861
% % b1_guided_tuned 39.0 https://tensorboard.corp.google.com/experiment/1926213812501357635/#timeseries
% % lr_guided_tuned 38.9
%%%%%%%%%%%%% OLD GREEDY BLEU
\begin{wraptable}{r}{8cm}
  \caption{Comparing BLEU scores of guided runs to baseline and the best of $100$ Bayesian-optimized runs across language pairs. Meta-learning-rate is set to $3\text{e-}5$ for untuned guided runs, and is tuned via BO in the final row.}% For the guided setting, the $4$ runs correspond to the coarse meta-learning rate tuning shown in Figures \ref{fig:beta1_sweep} and \ref{fig:lr_scalar_sweep}.}
  \footnotesize
  \centering
  \begin{tabular}{c|c|c|ccc}
    \toprule
    & BO-tuned & \# of runs & $\beta_1$ & $\alpha$ & $\beta_1$ \& $\alpha$\\
    \midrule
    \multirow{2}{*}{baseline} & no & 1 & 38.9 & 38.9 & 38.6 \\
     & yes &100 & 39.4 & 39.4 & 39.5 \\
    \midrule
    \multirow{2}{*}{guided} & no & 4 & 39.6 & 39.7 & \textbf{39.9} \\
    & yes &100 & 39.7 & 39.7 & \textbf{39.9} \\
    \bottomrule
  \end{tabular}
  \label{tab:tuned}
\end{wraptable}
% combo_base_single 38.55044937133789
% combo_base_tuned 39.462257385253906
% combo_guided_single 39.85588455200195
% combo_guided_tuned 39.85651397705078

% beta1_single_base 38.86009216308594
% beta1_tuned_base 39.43735885620117
% beta1_single_guided 39.76371383666992
% beta1_tuned_guided 39.60778045654297

% lr_single_base 38.86009216308594
% lr_tuned_base 39.3569450378418
% lr_single_guided 39.59181213378906
% lr_tuned_guided 39.73000717163086

\subsubsection{Analysis}

While the idea-scenario for guiding hyperparameters would involve no tuning of either the initialization or meta-learning-rate values, the \textit{short-horizon} problem faced by the learning rate necessitates tuning of the meta-learning-rate. However, for guided learning to be useful it simply needs to be a more efficient means of discovering useful hyperparameters than common HPO methods. In Figure \ref{fig:tuning} (and Table \ref{tab:tuned} we observe that guiding $\beta_1$, $\alpha$, or their combination actually outperforms Bayesian optimization (BO) in both absolute performance and in efficiency. Relative to BO with 100 training runs, guided learning achieves better results in each setting with a sweep over just 4 meta-learning-rate values. One potential reason is that the BO setup can only tune constant values, while the guided learning setup is capable of evolving hyperparameters over the course of training.%The optimal BO-tuned $\beta_1$ value is a constant $0.73$, which approximates the average value of the 

\subsection{Guiding T5}

In order to assess the extent to which our observations of guiding learning might generalize, we run similar experiments for T5 models. We run a guided experiments for $\beta_1$, $\alpha$, and the combination of the two. For $\beta_1$ alone, we replicate a similar converged schedule as in the NMR setting, but see only minor changes in accuracy across all models. For $\alpha$, we see the learning rate scalar plummet similarly to the NMT setting, but no guided run outperforms the baseline, even at mild meta-learning rates. For the combination of the two, we run a sweep over meta-learning rates and show results in Figure \ref{fig:t5}.


% % \begin{table}[h]
\begin{wraptable}{r}{7cm}
  \footnotesize
  \centering
  \begin{tabular}{c|c|ccccc}
    \toprule
    & base & \multicolumn{5}{c}{$\beta_1$ \& $\alpha$} \\
    $\hat{\eta}$ & - & $3\text{e-}6$ & $6\text{e-}6$ & $1\text{e-}5$ & $2\text{e-}5$ & $3\text{e-}5$ \\%& $4\text{e-}5$ \\
    \midrule
    \textit{acc} & 63.1 & 63.1 & \textbf{64.1} & \textbf{64.1} & 63.6 & 63.1 \\ %& 62.8 \\
    \textit{steps} & 1M & 1M & 600k & 440k & \textbf{290k} & 600k  \\%& - \\

    \bottomrule
  \end{tabular}
  \caption{Comparing final (1M steps) eval accuracy per token (\textit{acc)} and number of steps to reach baseline final accuracy (\textit{steps}) for a sweep of meta-learning rate values guiding $\alpha$ and $\beta_1$ for T5 models.}% The best-performing guided models improve by a full accuracy point, and the fastest-converging reaches the same performance as baseline in less than a third the number of steps.}
  \label{tab:t5}
\end{wraptable}
% i9_noguide 0.6311793
% combo_4e5 0.62831813
% combo_3e5 0.6310828
% combo_2e5 0.6363075
% combo_1e5 0.64058256
% combo_6e6 0.64078045
% combo_3e6 0.6311791

% ### appendix ###
% \begin{wrapfigure}{r}{0.5\textwidth}
%   \begin{center}
%     \includegraphics[width=0.48\textwidth]{draft_fig_t5.pdf}
%     \end{center}
%     \caption{Guiding learning rate scalar $\alpha$ and Adafactor's $\beta_1$ jointly for a T5 model, with runs color-coded by meta-learning rate.
%     }
% 	\label{fig:t5}
% \end{wrapfigure}
% % ### appendix ###

%The inter-dependence of hyperparameters is a huge barrier for multi-run hyperparameter tuning methods as the dimensionalisty of the search space grows linearly with the number of hyperparameters and the nature of interaction between different hyperparameters is unknown. In contrast to multi-run tuning methods, guided learning promises to be more powerful the more hyperparameters are simultaneously learned: as one guided parameter changes, it necessitates changes in the others which can be learned via the guidance loss. 

\subsubsection{Analysis}

Our T5 guided experiments on individual parameters replicate the parameter evolution seen in the NMT setting, but make only infinitesimal improvements over the baseline\footnote{See Appendix \ref{sec:appendix_t5} for figures.}. Interestingly, guiding both hyper-parameters simultaneously (Figure \ref{fig:t5}) appears to change the dynamics of their evolution to great effect, and we find a $3$X improvement in speed of convergence and significant increase in final performance for multiple different settings of meta-learning rate (Table \ref{tab:t5}). The plot of $\beta_1$ itself is familiar from the previous NMT experiments but the evolution of $\alpha$ takes on an complicated trajectory that appears related to the schedule of $\beta_1$. 

% The rough generalization of the guided ``recipe'' from NMT to T5 is encouraging for the possibility of finding generalized guided learning settings which perform well across domains. The demonstrated capacity to improve both speed and performance of T5 pretraining is a significant endorsement of the pragmatic value of the technique to improve over even well-tuned baselines. The superior performance of guiding the hyper-parameters jointly over each individually is a promising result and demonstrates a potential strategy for learning multiple kinds of hyper-parameters simultaneously.
% %That guiding the combination of hyper-parameters succeeds where guiding each individually fails is a hint as to both the promise and the complexity of learning multiple kinds of hyper-parameters simultaneously, and an obvious candidate for further exploration.

The rough generalization of the guided ``recipe'' from NMT to T5 is encouraging for the possibility of finding generalized guided learning settings which perform well across domains. The demonstrated capacity to improve both speed and performance of T5 pretraining is a significant endorsement of the pragmatic value of the technique to improve over even well-tuned baselines. The superior performance of guiding the hyper-parameters jointly over each individually is a promising and curious result that hints at both the potential and the complexity of learning multiple kinds of hyper-parameters simultaneously; an obvious candidate for further exploration. %. While non-gradient HPO techniques struggle to scale due to complex and unknown correlations between hyperparameters, this result suggests optimizing multiple kinds of hyper-parameters simultaneously via gradient methods may be much easier.
%That guiding the combination of hyper-parameters succeeds where guiding each individually fails is 



==> 5a_experiments.tex <==



\subsection{Guiding $\beta_1$}

In order to understand the function of guided learning we begin with a case study of a single hyperparameter, which yields a guided parameterization with only a single-dimensional degree of freedom. We start with $\beta_1$ as it is often useful to tune and is not complicated by the application of any schedule. In Figure \ref{fig:beta1_sweep}, we compare the evolution of $\beta_1$ over training for guided runs of differing meta-learning rates and initializations, training on the German-English language pair. The unguided baseline uses the default initialization of $0.9$. 
\begin{figure}
	\centering
    \includegraphics[width=\linewidth]{draft_fig_b1_sweep.pdf}
        \caption{Comparison of guiding $\beta_1$ over the course of training, with initialization values $[0.1,0.5,0.9]$ and meta-learning-rates [$3\text{e-}5$, $3\text{e-}4$, $3\text{e-}3$]. Baseline (no guidance) uses initialization of $0.9$ and meta-learning-rate of $0$. Loss on the development set and the learned $\beta_1$ values are shown in the top and bottom panels, respectively.}
	\label{fig:beta1_sweep}
\end{figure}


\subsection{Guiding $\alpha$}

We now explore the effects of tuning the learning rate ($\alpha$) via guided learning. Unlike $\beta_1$, the learning rate typically follows a predetermined schedule. Rather than throw away the benefits of the hard-coded scheme by training the learning rate value directly, we learn a scalar on the pre-defined schedule, i.e. $\textit{effective learning rate}_t = \textit{scalar} \times \textit{schedule}_t$. In Figure \ref{fig:lr_scalar_sweep} we show models trained on the German-English language pair, across guided runs coarsely tuning the learning rate scalar with varying meta learning rates.

\begin{figure}%[!htbp]
	\centering%
    \includegraphics[width=\linewidth]{draft_fig_lr_sweep.pdf}
        \caption{Learning rate scalars, color-coded by meta-learning rate. All guided runs are initialized at 1, and applied as a scalar to the same fixed learning rate schedule.}
	\label{fig:lr_scalar_sweep}
\end{figure}


\subsection{Combining guided parameters}
\begin{figure*}%[!htbp]
	\centering%
    \includegraphics[width=\linewidth]{draft_fig_combo.pdf}
        \caption{Comparing guiding runs to baseline across language-pairs (columns). Guided runs are the colored lines, the unguided baselines are black lines. The blue curves depict the guiding of the learning rate, the red that of $\beta_1$, and the purple, the combination of the two. The top row shows loss and the bottom shows accuracy on the development sets. All guided runs outperform all baseline runs in accuracy across language pairs.}
	\label{fig:language_pairs}
\end{figure*}
\begin{figure*}%[!htbp]
	\centering%
    \includegraphics[width=\linewidth]{draft_fig_vizier.pdf}
        \caption{Comparing guided runs for $\beta_1$ and learning rate in isolation and jointly, to unguided models, untuned and tuned, on the German-English language pair. The black solid line is the untuned baseline. The colored lines show a single guided run, learning the value of the variable(s) depicted at the top of the column. The dotted black lines show the best single run out of 100 produced in the course of an application of Bayesian optimization for tuning the variable(s) in question.}
	\label{fig:tuning}
\end{figure*}

Thus far we have analyzed guiding individual hyperparameters in isolation, holding the other hyperparameters constant. This simplifies the optimization problem and is helpful for analysis, but misses out on potential gains of jointly guiding parameters. In Figure \ref{fig:language_pairs}, we learn both $\beta_1$ and learning rate in a single run, setting the meta learning rate to $3\text{e-}5$ for both, and comparing against an un-guided baseline with default values across $6$ different language pairs. The max BLEU scores achieved per run are shown in Table \ref{tab:combo_bleu}.

\begin{table}[h]
  \caption{Comparing BLEU scores of guided runs to baseline across language pairs. Meta-learning-rate is set to $3\text{e-}5$ for all runs.}
  \footnotesize
  \centering
  \begin{tabular}{c|cccccc}
    \toprule
    & de-en & en-de & fi-en & en-fi & lt-en & en-lt \\
    \midrule
    baseline & 37.6 & 36.4 & 26.5 & 18.0 & 26.9 & 11.1 \\
    \midrule
    $\beta_1$ & \textbf{39.0} & \textbf{38.4} & \textbf{27.7} & 18.9 & \textbf{27.2} & 11.8 \\
    $\alpha$ & 38.8 & 38.3 & 27.0 & \textbf{19.3} & 27.1 & 11.4 \\
    $\beta_1$ \& $\alpha$ & 38.9 & \textbf{38.4} & 26.9 & 19.2 & 27.0 & \textbf{12.0} \\

    \bottomrule
  \end{tabular}
  \label{tab:combo_bleu}
\end{table}
% deen_combo_base 37.625935
% deen_beta1_glr3e5 39.000343
% deen_lr_glr3e5 38.75764
% deen_combo_glr3e5 38.86581

% ende_combo_base 36.445904
% ende_beta1_glr3e5 38.353165
% ende_lr_glr3e5 38.33833
% ende_combo_glr3e5 38.438854

% fien_combo_base 26.521357
% fien_beta1_glr3e5 27.66385
% fien_lr_glr3e5 27.030636
% fien_combo_glr3e5 26.937895

% enfi_combo_base 18.001335
% enfi_beta1_glr3e5 18.918892
% enfi_lr_glr3e5 19.25152
% enfi_combo_glr3e5 19.238531

% lten_combo_base 26.894577
% lten_beta1_glr3e5 27.234219
% lten_lr_glr3e5 27.059675
% lten_combo_glr3e5 27.034056

% enlt_combo_base 11.092238
% enlt_beta1_glr3e5 11.839374
% enlt_lr_glr3e5 11.373562
% enlt_combo_glr3e5 11.993965

\subsection{Comparing guidance to tuning}

In order to fairly evaluate the practical applicability of guiding these hyperparameters, it is necessary to compare the guided runs not just against the untuned baseline but against the best model produced by typical hyperparameter optimization schemes. This offers the opportunity to evaluate the relative utility of guidance vs tuning in terms of both absolute performance and efficiency. In Figure \ref{fig:tuning}, we compare guiding $\beta_1$, $\alpha$, and their combination against the best model (determined by the minimum of loss on the development set) produced by 100-model run of black-box optimization (BO) over the hyperparameter in question. We find that across guided-parameter settings, the non-BO-optimized guided run slightly outperforms the best BO-tuned model (Table \ref{tab:tuned}). For the setups which involve guiding $\alpha$, 
%which have more to gain from tuning due to the non-converging nature of guiding the learning rate, 
small additional gains are found in tuning the meta-learning rate with the same BO procedure.

\begin{table}[h]
  \caption{Comparing BLEU scores of guided runs to baseline and the best of $100$ Bayesian-optimized runs across language pairs. Meta-learning-rate is set to $3\text{e-}5$ for untuned guided runs, and is tuned via BO in the final row. For the guided setting, the $4$ runs correspond to the coarse meta-learning rate tuning shown in Figures \ref{fig:beta1_sweep} and \ref{fig:lr_scalar_sweep}.}
  \footnotesize
  \centering
  \begin{tabular}{c|c|c|ccc}
    \toprule
    & BO-tuned & \# of runs & $\beta_1$ & $\alpha$ & $\beta_1$ \& $\alpha$\\
    \midrule
    \multirow{2}{*}{baseline} & no & 1 & 38.0 & 38.0 & 38.0 \\
     & yes &100 & 38.6 & 38.7 & 38.8 \\
    \midrule
    \multirow{2}{*}{guided} & no & 4 & 39.0 & 38.8 & 38.9 \\
    & yes &100 & 39.0 & 38.9 & \textbf{39.1} \\
    \bottomrule
  \end{tabular}
  \label{tab:tuned}
\end{table}
% combo_base_single 37.625935
% combo_guided_single 38.86581
% combo_base_tuned 38.837517
% beta1_single_guided 39.11642
% beta1_single_base 38.045662

% beta1_tuned_base 38.561474
% lr_single_guided 38.81545
% lr_single_base 38.045662
% lr_tuned_base 38.7034


% combo_guided_tuned 39.1 https://xm2a.corp.google.com/experiments/33815861
% b1_guided_tuned 39.0 https://tensorboard.corp.google.com/experiment/1926213812501357635/#timeseries
% lr_guided_tuned 38.9


\subsection{Guiding T5}

In order to assess the extent to which our observations of guiding learning might generalize, we run similar experiments for T5 models. We run a guided experiments for $\beta_1$, $\alpha$, and the combination of the two. For $\beta_1$ alone, we replicate a similar converged schedule as in the NMR setting, but see only minor changes in accuracy across all models. For $\alpha$, we see the learning rate scalar plummet similarly to the NMT setting, but no guided run outperforms the baseline, even at mild meta-learning rates. For the combination of the two, we run a sweep over meta-learning rates and show results in Figure \ref{fig:t5}.

\begin{table}[h]
  \footnotesize
  \centering
  \begin{tabular}{c|c|cccccc}
    \toprule
    & base & $3\text{e-}6$ & $6\text{e-}6$ & $1\text{e-}5$ & $2\text{e-}5$ & $3\text{e-}5$ & $4\text{e-}5$ \\
    \midrule
    \textit{acc} & 63.1 & 63.1 & \textbf{64.1} & \textbf{64.1} & 63.6 & 63.1 & 62.8 \\
    \textit{steps} & 1M & 1M & 600k & 440k & \textbf{290k} & 600k  & - \\

    \bottomrule
  \end{tabular}
  \caption{Comparing final accuracy per token (\textit{acc)} and number of steps to reach baseline final accuracy (\textit{steps}) for a sweep of meta-learning rate values guiding $\alpha$ and $\beta_1$ for T5 models. The best-performing guided models improve by a full accuracy point, and the fastest-converging reaches the same performance as baseline in less than a third the number of steps.}
  \label{tab:t5}
\end{table}
% i9_noguide 0.6311793
% combo_4e5 0.62831813
% combo_3e5 0.6310828
% combo_2e5 0.6363075
% combo_1e5 0.64058256
% combo_6e6 0.64078045
% combo_3e6 0.6311791

\begin{figure}%[!htbp]
	\centering%
    \includegraphics[width=\linewidth]{draft_fig_t5.pdf}
        \caption{Guiding learning rate scalar $\alpha$ and Adafactor's $\beta_1$ jointly for a T5 model, with runs color-coded by meta-learning rate.
        }
	\label{fig:t5}
\end{figure}
%The inter-dependence of hyperparameters is a huge barrier for multi-run hyperparameter tuning methods as the dimensionalisty of the search space grows linearly with the number of hyperparameters and the nature of interaction between different hyperparameters is unknown. In contrast to multi-run tuning methods, guided learning promises to be more powerful the more hyperparameters are simultaneously learned: as one guided parameter changes, it necessitates changes in the others which can be learned via the guidance loss. 



==> 6_analysis.tex <==
\subsection{Guiding $\beta_1$}

Figure \ref{fig:beta1_sweep} illuminates the simplicity of the $\beta_1$ guidance-loss landscape; all runs with sufficiently high meta-learning rates converge\footnote{\textit{Convergence} in this sense can be observed in the gradients of the guided parameter, which settle towards $0$ for the runs which have reached the loss-defined optimum.} to remarkably similar schedules, regardless of model or $\beta_1$ initialization. That the different guided runs end up tracing the same schedule and that schedule outperforms not only the baseline, but even a thoroughly BO-tuned constant value, seems to realize a best-case scenario for guided learning: for optimizing $\beta_1$, expensive black-box optimization can be replaced with learning an optimal schedule with little or no tuning of the meta-learning rate.
%tuning $\beta_1$ can be done away with in favor of learning a better schedule with little or no tuning of the meta-learning rate at all.

Further, the converged $\beta_1$ schedule, which gently decreases $\beta_1$ over training, suggests a reasonable explanation. At the start of training, it is useful to have a high momentum as the peculiarities of the individual batches are less important than the general trends across them.
%(due to how little the model knows and how quickly it is progressing), but
As the model becomes better and training progress levels out, it is better to be sensitive to the peculiarities of the individual training batches rather than treating them all the same. A similar reasoning motivated early explorations of learning rate decay schedules \citep{lecun1991} and has been validated recently by \citet{you2019}. Thus analyzing the results from guided learning allows us to rediscover the intuitions that originally motivated exploration of learning rate decay schedules. %In doing so, we have demonstrated how a decay schedule can be successfully applied to $\beta_1$, a hyperparameter that is frequently tuned without a decay schedule.

Additionally, the 100-run Bayesian-optimized value of $\beta_1$ is roughly a constant approximation of the learned converged schedule, which is hardly changed by further BO-optimization\footnote{See Appendix \ref{sec:appendix} for plot.}. This suggests that the \textit{true optimal value} of the hyperparameter is following a schedule, and no amount of tuning a single constant value can beat a method that even roughly approximates that schedule. For hyperparameters whose optimal values change over training, methods that produce schedules will have an edge over global tuning methods (gradient-based or otherwise).

% This suggests a more general observation: if the optimal value of a hyperparameter follows a schedule over training rather than taking a single fixed value, then any global technique that selects a single constant value is at a disadvantage to methods (like greedy gradient-based optimization) which allow hyperparameters to take on a schedule of values. Picking the best constant value will lose to much less tuned schedules that are able to roughly approximate the optimal schedule.
%See Appendix TODO for gradients of converged and non-converged runs from Figure \ref{fig:beta1_sweep}.}
% Of course this only follows if the converged schedule is actually better! In Figure \ref{fig:beta1_sweep} we show the losses of each run on the development set, and observe that all guided models outperform the baseline model. The observation that many of the guided runs achieve similar performance, despite the two orders of magnitude difference in their meta-learning rate values, demonstrates that when guided parameters converge, tuning the meta-learning rate is a much more forgiving task than tuning the parameters themselves.


% This case study has demonstrated the possibility of learning a schedule for $\beta_1$ with little or no tuning that offers significant efficiency gains over traditional multi-run static tuning, as well as performance improvement over the best tuned setup. The gradually decaying schedule learned for $\beta_1$ is reminiscent of common learning-rate decay schedules. Naturally, we now perform the same analysis on the learning rate - often the single most important hyperparameter.

\subsection{Guiding learning rate}
It is crucial to tune the learning rate and its schedule to achieve good results \cite{Bengio2012}. Unfortunately tuning a schedule is a much more complicated task than tuning a single constant value, so in practice (including in this work), learning rate schedules are frequently borrowed from previous work. 
%The importance of the learning rate schedule coupled with the frequency with which it is copied from prior art without additional tuning implies headroom for improved performance with careful schedule tuning, gated only by the prohibitive complexity of tuning the learning rate with extant methods. 
 \cite{wu2018understanding} have shown that learning the learning rate greedily is subject to a \textit{short-horizon bias}, whereby the gradient of the guidance loss drives the learning rate too low and thus fails to actually learn, yielding a worse final model. This position is supported by the results of our sweep over meta-learning rates for guiding $\alpha$ (Figure \ref{fig:lr_scalar_sweep}), in which the run with the highest meta-learning rate ($3\text{e-}3$) spikes initially and then decays quickly to convergence at a nearly static value of $1\text{e-}5$ for the rest of training. This short-horizon bias means that unlike $\beta_1$, the meta-learning rate cannot simply be set to a high-enough value for convergence, but must be tuned if it is to help performance. 

However, even with a modest sweep over meta-learning rates, we are able to substantially outperform the baseline schedule. Indeed we are even able to surpass the best result from a much more expensive Bayesian optimization of the non-guided learning rate. This suggests that tuning the meta-learning rate may still be a more pragmatic approach to optimization rather than tuning the original learning rate.

\subsection{Combination and Generalization}
In Figure \ref{fig:language_pairs}, we observe that guided learning of $\beta_1$, $\alpha$, or the combination of the two outperforms the baseline across language pairs, which suggests that it may be possible to find ``good recipes'' which generalize across training runs, further simplifying the useful application of guiding hyperparameters. While guiding $\beta_1$ and $\alpha$ together doesn't drastically change the dynamics of their evolution compared to learning each alone, we find that in some cases the combination of the two yields better results than guiding them separately, and when tuned, they outperform the individual setups.
% One of the difficulties for per-training-run HPO when optimizing multiple hyperparameters simultaneously is disentangling correlations between concurrently tuned hyperparameters. Learning hyperparameters online offers an opportunity to turn this correlation into an advantage by allowing guided parameters to dynamically adjust to the other hyperparameters, even as those may also be changing. In our experiments combining learning $\beta_1$ and $\alpha$ we did not observe any difference in the evolution of each guided parameter compared to the single-guided-parameter setting, but we do 

\subsection{Guidance vs Tuning}
While the idea-scenario for guiding hyperparameters would involve no tuning of either the initialization or meta-learning-rate values, the \textit{short-horizon} problem faced by the learning rate necessitates tuning of the meta-learning-rate. However, for guided learning to be useful it simply needs to be a more efficient means of discovering useful hyperparameters than common HPO methods. In Figure \ref{fig:tuning} (and Table \ref{tab:tuned} we observe that guiding $\beta_1$, $\alpha$, or their combination actually outperforms Bayesian optimization (BO) in both absolute performance and in efficiency. Relative to BO with 100 training runs, guided learning achieves better results in each setting with a sweep over just 4 meta-learning-rate values. One potential reason is that the BO setup can only tune constant values, while the guided learning setup is capable of evolving hyperparameters over the course of training.%The optimal BO-tuned $\beta_1$ value is a constant $0.73$, which approximates the average value of the 

\subsection{Guiding T5}
Our T5 guided experiments on individual parameters replicate the parameter evolution seen in the NMT setting, but make only infinitesimal improvements over the baseline\footnote{See Appendix \ref{sec:appendix_t5} for figures.}. Interestingly, guiding both hyper-parameters simultaneously (Figure \ref{fig:t5}) appears to change the dynamics of their evolution to great effect, and we find a $3$X improvement in speed of convergence and significant increase in final performance for multiple different settings of meta-learning rate (Table \ref{tab:t5}). The plot of $\beta_1$ itself is familiar from the previous NMT experiments but the evolution of $\alpha$ takes on an complicated trajectory that appears related to the schedule of $\beta_1$. 

% The rough generalization of the guided ``recipe'' from NMT to T5 is encouraging for the possibility of finding generalized guided learning settings which perform well across domains. The demonstrated capacity to improve both speed and performance of T5 pretraining is a significant endorsement of the pragmatic value of the technique to improve over even well-tuned baselines. The superior performance of guiding the hyper-parameters jointly over each individually is a promising result and demonstrates a potential strategy for learning multiple kinds of hyper-parameters simultaneously.
% %That guiding the combination of hyper-parameters succeeds where guiding each individually fails is a hint as to both the promise and the complexity of learning multiple kinds of hyper-parameters simultaneously, and an obvious candidate for further exploration.

The rough generalization of the guided ``recipe'' from NMT to T5 is encouraging for the possibility of finding generalized guided learning settings which perform well across domains. The demonstrated capacity to improve both speed and performance of T5 pretraining is a significant endorsement of the pragmatic value of the technique to improve over even well-tuned baselines. The superior performance of guiding the hyper-parameters jointly over each individually is a promising and curious result that hints at both the potential and the complexity of learning multiple kinds of hyper-parameters simultaneously; an obvious candidate for further exploration. %. While non-gradient HPO techniques struggle to scale due to complex and unknown correlations between hyperparameters, this result suggests optimizing multiple kinds of hyper-parameters simultaneously via gradient methods may be much easier.
%That guiding the combination of hyper-parameters succeeds where guiding each individually fails is 


==> 7_future_work.tex <==
% TODO

==> 8b_limitations.tex <==
% Limitations

% In running the same experiments for NMT and T5, we've attempted to assess 

% We've attempted to assess the function and generlizability of learning two specific hyper-parameters for sequence-to-sequence models. 

% In this work, we've applied a greedy gradient-based method to learn hyper-parameters during training. We've shown that greedily learning $\beta_1$ is not susceptible to the `short-horizon bias', and can learn a schedule which out-performs optimal constant-valued tuning. For NMT, we've shown that tuning the meta-hyper-parameter \mlr{} while learning either $\alpha$ or $\beta_1$ is much more efficient than tuning the hyper-parameters themselves. In the T5 pretraining setting, we've demonstrated that learning the hyper-parameters together can change the dynamics of their evolution. The 

Our experiments are limited to two global hyper-parameters which are typically tuned. Future work should explore a wider set of hyper-parameters and at a finer granularity (eg. a distinct hyper-parameter value per parameter, as in \cite{lorraine2020}). We show that learning hyper-parameters together can alter their dynamics but leave to future work the characterization of the mechanism and mapping of interactions between learned hyper-parameters. We show that learning isolated hyper-parameters can improve performance with less tuning than typical methods for NMT, but that 
